Complementary Benefits of Contrastive Learning and Self-Training Under Distribution Shift

Self-training and contrastive learning have emerged as leading techniques for incorporating unlabeled data, both under distribution shift (unsupervised domain adaptation) and when it is absent (semi-supervised learning). However, despite the popularity and compatibility of these techniques, their efficacy in combination remains unexplored. In this paper, we undertake a systematic empirical investigation of this combination, finding that (i) in domain adaptation settings, self-training and contrastive learning offer significant complementary gains; and (ii) in semi-supervised learning settings, surprisingly, the benefits are not synergistic. Across eight distribution shift datasets (e.g., BREEDs, WILDS), we demonstrate that the combined method obtains 3--8% higher accuracy than either approach independently. We then theoretically analyze these techniques in a simplified model of distribution shift, demonstrating scenarios under which the features produced by contrastive learning can yield a good initialization for self-training to further amplify gains and achieve optimal performance, even when either method alone would fail.

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}


Self-training and contrastive pretraining are two common approaches for incorporating unlabeled data in machine learning. These methods were initially proposed as techniques for semi-supervised learning (SSL), in which the aim is to use a small set of labeled and large set of unlabeled data to achieve good in-distribution performance. However, they have also become strong baselines for unsupervised domain adaptation (UDA), a scenario where there is a shift in distribution between source and target, and the goal is to learn a classifier that achieves good out-of-distribution performance using only source labeled data and target unlabeled data.

At a high level, self-training methods work by  first learning a predictor using source labeled data, and then propagating labels from the source predictor onto unlabeled target (pseudolabels) and overfitting the predictor to the pseudolabeled data. 
Methods for contrastive pretraining instead learn representations on unlabeled data (from both source and target) by enforcing invariance to augmentations, which extracts features that effectively identify clusters of data points in the augmentation graph~\citep{haochen2021provable}.  Motivated by the strong empirical performance of these 
methods, several recent works have  attempted to understand 
the behavior of these 
approaches~\citep{wei2020theoretical, haochen2021provable, saunshi2022understanding, shen2022connect, cai2021theory, haochen2022beyond, haochen2022theoretical, cabannes2023ssl}.
However, despite these efforts, there is no common consensus on 
whether self-training or contrastive pretraining should be employed 
given a pool of target unlabeled data. 
Moreover, since both methods utilize unlabeled data in distinct ways, 
it remains unclear (both empirically and theoretically) 
whether benefits derived from these approaches are complementary.



















In this paper, we address this gap by investigating the 
complementary nature of self-training 
and contrastive pretraining. 
Surprisingly, we find that while self-training  over contrastive pretraining yields negligible gains for SSL (labeled data is from the same distribution as unlabeled), self-training over contrastively pretrained representations provides significant gains in out-of-distribution performance for UDA (unlabeled data from shifted distribution). 
In particular, our findings across ten distribution shift datasets show that re-using target unlabeled data for self-training over representations that were contrastive-learned using unlabeled from source and target  yields $\approx5$\% improvement on average OOD performance (UDA) as opposed to $<0.8\%$ 
average improvement on ID performance in SSL setups (Figure XX). We then explore this behavior theoretically by analyzing the combined benefits of XX. Overall, we make the following contributions:
...
\gs{Add contribution list?}
\gs{Cut everything below this, or move to related work section?}

In this paper, we address this gap by investigating the 
complementary nature of self-training 
and contrastive pretraining. 
Surprisingly, we find that while self-training 
over contrastive pretraining yields negligible gains in ID performance for SSL (labeled data is from the same distribution as unlabeled), self-training over contrastively pretrained representations provides significant gains in OOD performance for UDA (unlabeled data from shifted distribution). 
Accumulating findings on ten distribution shift datasets (including BREEDs datasets~\citep{santurkar2020breeds}, 
FMoW-WILDs~\citep{wilds2021}, Visda~\citep{visda2017} and OfficeHome~\citep{venkateswara2017deep}), we observe that re-using target unlabeled data for self-training (FixMatch algorithm~\citep{sohn2020fixmatch}) over representations that were contrastive learned (SwAV~\citep{caron2020unsupervised}) using unlabeled from source and target, 
yields $\approx5$\% improvement on average OOD performance (UDA) as opposed to $<0.8\%$ %
average improvement on ID performance in SSL setups. 
Additionally, to understand the performance ceiling of contrastive 
representations on target data, 
we obtain linear probed heads (fixing representations) separately with 
source and target labeled data. 
We find that head trained on target has $>20\%$ OOD accuracy compared to head trained on source, which tells us that while the features are good the linear probed head on source does not generalize OOD on target. However, when we subsequently self-train over this we can bridge approximately half of the gap. 
This is somewhat surprising in the context of existing theoretical works for UDA that attribute transferability of linear heads (from source to target) to contrastive pretraining~\citep{shen2022connect,haochen2022beyond}.  

















\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.6\linewidth]{images/figure1a-light.pdf} \hfill 
    \color{gray}\vrule width 0.03cm{} \hfill
    \includegraphics[width=0.38\linewidth]{images/CLST_fig1_horizontal.pdf} 
    \caption{Caption \sg{(i) Make FT to ERM, CL+FT to CL and keep others the same, (ii) Add shift and no shift in SSL and UDA acroynm in the plot; (iii) Update Figure 3 with the suggestions AR made (almost done!)}}
    \label{fig:figure-one}
\end{figure*}




\emph{Why self-training improves over contrastive learning under distribution shifts?} 
To answer this, consider a distribution shift setting that includes two types of features: 
(i) invariant features that perfectly predict the label, and (ii) domain-dependent features that are predictive of the label in either just source or target (spurious correlations). 
Our theoretical analysis reveals that contrastive pretraining on unlabeled data identifies clusters realized by both domain-dependent and invariant features.
Consequently, when we train a linear head on these representations using just source labeled data, the classifier relies on domain-dependent features (from source) and fails to generalize OOD on target.
Nevertheless, contrastive pretraining does provide  a ``good'' initialization for self-training, \ie, in essence the representations rely less on domain dependent features---effectively amplifying invariant features in the representation space (as compared to raw source data)
Now,  while the linear probed head still does not generalize OOD it  provides ``good'' initial pseudolabels on the target unlabeled data.  
As a result, self-training on top of contrastive learned features effectively unlearns the reliance on domain-dependent features and generalizes perfectly OOD.
Our analysis also demonstrates that when self-training is done from scratch (directly on the data and not on pretrained representations), it fails to generalize OOD since the pseudolabels are obtained through a predictor that mainly relies on domain-dependent features. Now, iterative self-training may not eliminate dependence on such features (in fact it escalates it) and could converge to a classifier with near-random OOD performance.
In contrast, for SSL settings 
(\ie, in distribution), 
our analysis highlights that contrastive pretraining already acquires sufficient predictive features 
such that linear probing (with a small amount of) labeled data attains near-optimal ID generalization. Hence, there is not much to gain from self-training over this in SSL.



















\ar{Sounds more like a zoom issue, rather than what you were going for :) Maybe challenges? }
\ar{This whole paragraph was extremely difficult for me to parse... I think you should assume that the readers would expect the intro to be easy to read, so try to explain the differences with prior work in a more understandable way}
\textbf{Technical difficulties~~}         
Existing theoretical work on understanding self-training and contrastive pretraining
focuses on the augmentation graph of the unlabeled 
data~\citep{arora2019theoretical, wei2020theoretical, haochen2021provable, johnson2022contrastive, saunshi2022understanding, garrido2022duality, haochen2022theoretical}. \ar{What should I take away from this statement?}
\newline
\ar{Different abstract assumptions between CL and ST; lack of distribution shift in CL literature, source classifier error for analysing ST, but not clear how the source classifier is obtained }
\emph{(i)~Contrastive pretraining challenges:} \todosg{unclear if emph is ok? Bold was too much bold :p}
Existing theories make 
assumptions where data augmentations implicitly encode 
label information for the downstream task.
Building on these assumptions, 
recent papers show that contrastive pretraining methods 
learn representations that linearly transfer under distribution shift~\citep{haochen2022beyond, shen2022connect, cabannes2023ssl}. 
However, we observe that in practice, 
while contrastive pretraining (on union on source and target data) 
learns ``somewhat'' transferable features, 
the difference in average accuracy on the target (in our testbed) between 
linear probing with target data and linear probing with labeled source data is $>20\%$.
These empirical findings call into question 
existing assumptions on data augmentations, highlighting that
perfect linear transferability may not typically hold in practice. 
\newline
\emph{(ii)~Self-training challenges:} 
On the other hand, the majority of previous studies 
analyzing self-training focus on consistency loss by making 
an expansion assumption regarding the data distribution 
and augmentations~\citep{cai2021theory, wei2020theoretical}. 
However, even when this assumption is satisfied, 
iteratively optimizing the consistency loss (even in population) 
can be challenging and will depend on the 
sampling frequency of ``favorable'' augmentations. 
We highlight and discuss the failures arising from 
iterative optimization in our toy setup.
\todosg{Add a note on how this relates to our setup.}
These findings emphasize the need for iterative analysis 
in self-training, similar to \citep{chen2020self}, instead of analyzing consistency 
loss and its global minimizer. 
Moreover, to the best of our knowledge, a unified framework to 
study self-training and contrastive pretraining is also 
absent in the literature. 
\newline
{To tackle these challenges}, we show that the 
behavior resembling our empirical findings
on real-world data emerges even in a simple toy setup.
\ar{Not clear how just having a toy setup addresses all the challenged above}
We conduct a theoretical analysis of two-layer linear networks. 
After obtaining a closed-form solution 
for the contrastive pretraining objective, 
our analysis examines the conditions on  
the initialization under which 
population iterates of self-training converge 
to an optimal target classifier. 
\ar{Right now you only make it clear that prior work doesn't get what we want, but it doesn't say how exactly you address the challenges..In which case, it's better suited for related work. But if you really want to talk about technical contributions in the intro, it has to be done differently}












\textbf{Algorithmic implications~~} 
In the context of SSL, 
contrastive pretraining (and more generally self-supervised methods) 
has become a de-facto method of choice~\red{cite}. 
Meanwhile, for DA, both self-training and 
contrastive learning methods have individually 
demonstrated promise in existing benchmarks~\red{cite}. 
Our analysis reveals an intuitive story that under distribution shift, 
the same unlabeled target data can be leveraged to \emph{not only 
improve representation learning but also  
improve the classifier learning on top}, thereby 
increasing the linear transferability of those representations. 
It's important to note that we are not claiming that self-training over contrastive pretraining 
to be a SOTA method. To summarize, the primary contribution of our work are: 
(i) identifying the phenomenon that self-training 
can significantly improve over contrastive pretraining under distribution shift; 
and (ii) analyzing and providing intuitions on why this phenomenon emerges. 
We hope that our analysis inspires future work to improve methods for UDA.




==> sections/introduction_may12.tex <==
\section{Introduction}
\label{sec:intro}
\ar{I would recommend a slightly different structure where the experimental results come before---that's very exciting. Then motivate that we want to understand this better, and then talk about why prior work doesn't give us a simple way to do this. We provide insight and along the way build up some new tools or analysis...Then talk about other potential insights or tests we can do about our theory. I wouldn't put the FixMatch + Contrastive under empirical validation...loses signficance that way}

\ar{Overall, in the first paragraph, it's a bit unclear what points exactly you are trying to make...it might be useful to think about what broader context you want to set, and what's really relevant or important for motivating the paper.}
When deployed in real-world settings, machine learning models 
frequently face distribution shift issues, where the 
deployment data exhibits \ar{What qualifies as a statistical difference?} statistical differences from the training data~\citep{quinonero2008dataset, 
torralba2011unbiased, wilds2021}. 
\ar{The shift is not the issue---the drop in performance is the issue}
Continuous data labeling \ar{this doesn't follow from the previous sentence} can be prohibitively costly, 
prompting researchers to focus on Unsupervised Domain Adaptation (UDA). 
In this setting, given only labeled data from the source distribution and unlabeled data from the target distribution, the goal is to learn a target domain classifier. \ar{What is a target domain classifier? You mean a classifier that performs well on the target domain?}
Since the UDA problem is underspecified without assumptions 
about the nature of the shift~\citep{ben2010impossibility}, 
researchers have traditionally explored additional assumptions 
that render the problem well-posed~\citep{shimodaira2000improving, scholkopf2012causal}.  
An alternative prominent research approach focuses on developing 
heuristics that profitably incorporate unlabeled target data on benchmark datasets, 
which capture the kinds of 
distribution shift that appear in practice, e.g., 
BREEDs~\citep{santurkar2020breeds}, Officehome~\citep{venkateswara2017deep}, 
WILDS~\citep{wilds2021}. 
\ar{I'm confused---if UDA (with access to unlabeled target data) is underspecified, how can heuristics that incoroporate unlabeled data help? I think I see what you're trying to say, but it should be conveyed better. Also not clear, if you really need it.}


Self-training~\citep{sohn2020fixmatch, xie2020self, wang2021tent} and contrastive pretraining approaches~\citep{caron2020unsupervised, chen2020simple, zbontar2021barlow}---initially proposed for Semi-Supervised Learning (SSL) where the unlabeled data distribution aligns with the covariate distribution in labeled data---have emerged as strong empirical baselines for  
UDA~\citep{sagawa2021extending, garg2022RLSbench, cai2021theory, shen2022connect}. 
\ar{This next paragraph is an important one. Has to be written more carefully and precisely.}
Self-training methods utilize unlabeled data to propagate labels across 
different augmentations \ar{not clear that the augmentations are on the unlabeled data. It is also not standard for self-training to depend on augmentations..Usually, it's just pseudolabels on unlabeled data..} while minimizing errors on labeled data. \ar{Not sure where the minimizing errors on labeled data came from...this sounds like source labeled data but that's probably not what yo meant..} 
In contrast, contrastive learning methods learn 
representations by enforcing clustering of augmentations of unlabeled data, \ar{again, this is not how people usually think of contrastive learning..} 
and subsequently, a classifier is trained on labeled data 
using these representations, often through linear probing.
Motivated by the strong empirical performance of these 
methods, several recent research attempts have been essayed to understand 
the behavior of these 
approaches~\citep{wei2020theoretical, haochen2021provable, saunshi2022understanding, shen2022connect, cai2021theory, haochen2022beyond, haochen2022theoretical, cabannes2023ssl}.
However, despite these efforts, there is no common consensus on 
whether self-training or contrastive should be employed 
given a pool of target unlabeled data. 
Moreover, since both methods utilize unlabeled data in distinct ways, 
it remains precariously underexplored (both empirically and theoretically) 
whether the benefits derived from these approaches are complementary.

In this paper, we address this gap by investigating the 
complementary nature of self-training 
and contrastive pretraining. 
Surprisingly, we find that while self-training 
over contrastive pretraining yields a small 
(to negligible) gain in performance in SSL \ar{seems important to remind people what SSL is; and you wrote the initial paragraph about UDA, so it's unclear where the SSL came from} problems, self-training can provide 
significant gains over contrastively pretrained 
models in the presence of distribution shifts.
\ar{Probably want to add some concrete results here}




\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.4\linewidth]{images/fig-1-left.jpeg}
    \includegraphics[width=0.3\linewidth]{images/fig-1-center.jpeg}    
    \includegraphics[width=0.25\linewidth]{images/fig-1-right.jpg}    
    \caption{Caption}
    \label{fig:figure-one}
\end{figure*}



\emph{Why self-training improves over contrastive learning under distribution shifts?} 
\ar{The current writing somehow doesn't inspire me to really think about this question...}
\ar{Domain-independent and domain-dependendent are somewhat non standard terms, so maybe explain that a bit with some concrete example}
\ar{I would try to frame this as "We consider a distribution shift setting with two types of features..., because we haven't proved that this is the only type of shift that exhibits the trends of interest}
Our theoretical analysis reveals that if the distribution 
shift setup includes two types of features: 
(i) domain-invariant features that perfectly predict 
the label, and (ii) domain-dependent features predictive 
of label only in the source domain, 
then the contrastively pretraining representations 
\emph{provably} depend  on domain-dependent features.
\ar{I first read it as domain-independent... I think this paragraph can also be improved by explaining things carefully while being simple yet precise}
Consequently, subsequent linear probing with 
source labeled data
\emph{cannot} produce an optimal target classifier.
However, contrastive pretraining does provide 
a ``good'' initialization, \ie, in essence 
the representations have a reduced dependence 
on domain-dependent features (compared to 
training from scratch), such that 
linear probing on the source
provides ``good'' pseudolabels 
on the target.  
\ar{It would be good to establish terminology that's shared across the intro and paper.. for .e.g. we didn't talk about pseudolabels when discussing self training before}
As a result, self-training in the second stage 
effectively unlearns the reliance on domain-dependent 
features and recovers an optimal target classifier.
Our analysis also demonstrates that self-training, 
when performed after training on source-labeled data 
from scratch, is inadequate, as iterative self-training 
may not eliminate the domain-dependent 
features and could converge to a classifier 
with near-random target performance.
\ar{Previous sentence was very dense}
In contrast, for SSL settings 
(\ie, in distribution), 
our theory highlights that contrastive pretraining 
acquires sufficient discriminative features 
such that linear probing (with a small 
amount of) labeled data attains near-optimal performance.





\ar{Sounds more like a zoom issue, rather than what you were going for :) Maybe challenges? }
\ar{This whole paragraph was extremely difficult for me to parse... I think you should assume that the readers would expect the intro to be easy to read, so try to explain the differences with prior work in a more understandable way}
\textbf{Technical difficulties~~}         
Existing theoretical work on understanding self-training and contrastive pretraining
focuses on the augmentation graph of the unlabeled 
data~\citep{arora2019theoretical, wei2020theoretical, haochen2021provable, johnson2022contrastive, saunshi2022understanding, garrido2022duality, haochen2022theoretical}. \ar{What should I take away from this statement?}
\newline
\emph{(i)~Contrastive pretraining challenges:} \todosg{unclear if emph is ok? Bold was too much bold :p}
Existing theories make 
assumptions where data augmentations implicitly encode 
label information for the downstream task.
Building on these assumptions, 
recent papers show that contrastive pretraining methods 
learn representations that linearly transfer under distribution shift~\citep{haochen2022beyond, shen2022connect, cabannes2023ssl}. 
However, we observe that in practice, 
while contrastive pretraining (on union on source and target data) 
learns ``somewhat'' transferable features, 
the difference in average accuracy on the target (in our testbed) between 
linear probing with target data and linear probing with labeled source data is $>20\%$.
These empirical findings call into question 
existing assumptions on data augmentations, highlighting that
perfect linear transferability may not typically hold in practice. 
\newline
\emph{(ii)~Self-training challenges:} 
On the other hand, the majority of previous studies 
analyzing self-training focus on consistency loss by making 
an expansion assumption regarding the data distribution 
and augmentations~\citep{cai2021theory, wei2020theoretical}. 
However, even when this assumption is satisfied, 
iteratively optimizing the consistency loss (even in population) 
can be challenging and will depend on the 
sampling frequency of ``favorable'' augmentations. 
We highlight and discuss the failures arising from 
iterative optimization in our toy setup.
\todosg{Add a note on how this relates to our setup.}
These findings emphasize the need for iterative analysis 
in self-training, similar to \citep{chen2020self}, instead of analyzing consistency 
loss and its global minimizer. 
Moreover, to the best of our knowledge, a unified framework to 
study self-training and contrastive pretraining is also 
absent in the literature. 
\newline
{To tackle these challenges}, we show that the 
behavior resembling our empirical findings
on real-world data emerges even in a simple toy setup.
\ar{Not clear how just having a toy setup addresses all the challenged above}
We conduct a theoretical analysis of two-layer linear networks. 
After obtaining a closed-form solution 
for the contrastive pretraining objective, 
our analysis examines the conditions on  
the initialization under which 
population iterates of self-training converge 
to an optimal target classifier. 
\ar{Right now you only make it clear that prior work doesn't get what we want, but it doesn't say how exactly you address the challenges..In which case, it's better suited for related work. But if you really want to talk about technical contributions in the intro, it has to be done differently}








\ar{My personal preference is to have experiments before the theory... i feel it dilutes the experimental contribution to make it a "validation".. the truth is we did the reverse and I think that's more compelling... related to my comment earlier on being more concrete about the results right when you said that we find these approaches complementary for UDA.}
\textbf{Experimental validation~~}
We experiment with $10$ vision
distribution shift datasets (including 4 BREEDs datasets~\citep{santurkar2020breeds}, 
FMoW-WILDs~\citep{wilds2021}, Visda~\citep{visda2017} and OfficeHome~\citep{venkateswara2017deep}).
For contrastive pretraining, we perform SwAV~\citep{caron2020unsupervised}
 with the union of source and target unlabeled data
and for self-training, we implement the FixMatch algorithm~\citep{sohn2020fixmatch}. 
For SSL, we perform 
experiments with the source datasets 
by simply reducing the amount of labeled data. 
First, we observe that self-training and contrastive pre-training 
together yield >8\% improvement on average target performance
under distribution shift as opposed to <1\% average improvement
in SSL setups. 
Second, to understand the performance ceiling of contrastive 
representations on target data, 
we train linear probes (fixing representations) separately with 
source and target labeled data. 
We observe $>20\%$ gap in performance on the target data,
and we observe that self-training subsequently 
bridges approximately half of the gap. 



\textbf{Algorithmic implications~~} 
In the context of SSL, 
contrastive pretraining (and more generally self-supervised methods) 
has become a de-facto method of choice~\red{cite}. 
Meanwhile, for DA, both self-training and 
contrastive learning methods have individually 
demonstrated promise in existing benchmarks~\red{cite}. 
Our analysis reveals an intuitive story that under distribution shift, 
the same unlabeled target data can be leveraged to \emph{not only 
improve representation learning but also  
improve the classifier learning on top}, thereby 
increasing the linear transferability of those representations. 
It's important to note that we are not claiming that self-training over contrastive pretraining 
to be a SOTA method. To summarize, the primary contribution of our work are: 
(i) identifying the phenomenon that self-training 
can significantly improve over contrastive pretraining under distribution shift; 
and (ii) analyzing and providing intuitions on why this phenomenon emerges. 
We hope that our analysis inspires future work to improve methods for UDA.




==> sections/problemsetup.tex <==
In this section, we formally describe the task and metrics of interest, and then define the various objectives for learning from labeled and unlabeled data.
We use $\|\cdot\|_2$ for $l_2$ and $\|\cdot\|_F$ Frobenius norm. 
\paragraph{Task.} Our goal is to learn a predictor that maps inputs $x \in \R^d$ to outputs $y \in \sY = \{1, 2, \hdots k\}$. We parameterize predictors $f_\theta: \sX \mapsto \sY$ as $\argmax H_\theta \Phi_\theta$ where $\Phi_\theta:\sX \mapsto \R^d$ is a feature map and $H_\theta \in \R^{k \times d}$ is a linear classifier that maps the representation to the final scores or logits. We drop the subscript $\theta$ for notational convenience. 

Let $\ProbS, \ProbT$ be the source and target joint probability measures over $\inpt\times\out$ with $\ps$ and $\pt$ as the corresponding probability density (or mass) functions. We are given labeled samples from the source, and a much larger unlabeled pool drawn from a mixture of source and target data. Unlabeled data is typically much cheaper to obtain, and our goal is to leverage this along with a few labeled source data to achieve good performance on the target distribution.

Formally, given access to labeled samples $(x_1, y_1), \hdots (x_n, y_n) \sim \ProbS$ and unlabeled samples $x_1, \hdots x_m \sim \ProbU = (1/2)\cdot \ProbS(x) + (1/2) \cdot \ProbT(x)$, our goal is to learn a classifier $f_\theta$ with low target error defined as follows: 
\begin{align*}
\targeterr(\theta) = \mathbb{E}_\ProbT[\argmax f_\theta(x) \neq y]
\end{align*}
We study two particular instances: (i) Unsupervised domain adaptation (UDA) and (ii) Semi-supervised learning (SSL). In UDA, we assume that the source and target distributions have the same label marginals $\ProbS(y) = \ProbT(y)$ (i.e. no label shift) and the same Bayes optimal predictor, \ie, $\argmax_y \ps(y \mid x) = \argmax_y \pt(y \mid x)$. In SSL, there is no distribution shift and $\ProbS=\ProbT=\ProbU$. 

\todosg{Amrith I made some edits, I have cached your version below, you can change accordingly. }





\paragraph{Methods.} 
\ar{This is not the place you want to save space...it's important to explain this part properly. Left it to you to create appropriate macros for different methods}
\begin{enumerate}[leftmargin=*]
    \item Source-only ERM (ERM): A standard approach is to simply perform supervised learning on the labeled source data by minimizing the empirical risk $\sum \limits_{i=1}^n \ell(H_\theta \Phi_\theta(x), y)$, for some classification loss $\ell$ (e.g. cross entropy). 
    \item Contrastive Learning (CL): In CL, we first use the unlabeled data to learn a good feature extractor. In particular, the objective is to learn a feature extractor $\Phi_\cl$ that maps augmentations (for e.g. crops or rotations) of the same input close to each other and far from augmentations of random other inputs \cite{caron2020unsupervised, chen2020simple, zbontar2021barlow}. Once we have $\Phi_\cl$, we learn a linear classifier $H_\theta$ on top to minimize a classification loss on the labeled source data. We could either keep $\Phi_\cl$ fixed or propagate gradients through.  
    \item Self-training (ST): This is a two stage procedure, where the first stage performs source-only ERM by just looking at source labeled data. In the second stage, we iteratively apply the current classifier on the unlabeled data to generate ``pseudo-labels'' and then update the classifier by minimizing a classification loss on the pseudolabeled data \citep{lee2013pseudo}.  
\ar{Move the exact fixMatch to experiment section detail}
\item Combining contrastive and self-training (CL + ST). Finally, a natural extension of the approaches above is the following: rather than starting with a source-only ERM classifier, one could perform the second stage of self-training initialized with a CL classifier instead. The CL classifier has already used the unlabeled data in learning the feature representation, but ST further continues to use the same unlabeled data to propagate pseudolabels. As we identify experimentally and theoretically, combining the two unsupervised objectives improves substantially over each method independently.
\end{enumerate}
































































==> sections/theory_bkup_oct15.tex <==
\vspace{-5pt}
\section{Theoretical Analysis and Intuitions}
\vspace{-5pt}
\label{sec:theory}

Our results on real-world datasets 
suggest that although self-training may offer 
little to no improvement over contrastive pretraining 
for in-distribution (\ie, SSL) settings, 
it leads to substantial improvements 
when facing distribution shifts in UDA (\secref{sec:exp}). 
Why do these methods offer complementary gains, 
but only under distribution shifts? 
In this section, we seek to answer this question 
by first replicating all the empirical trends of interest 
in a simple data distribution with an intuitive story (\secref{subsec:intuitive-story}). 
In this toy model, we formally characterize the gains afforded 
by contrastive pretraining and self-training both individually 
(Secs. \ref{subsec:self-training-analysis}, \ref{subsec:contrastive-pretraining-analysis}) 
and when used together 
(\secref{subsec:combining-self-training-and-contrastive-pretraining}).
 

\newcommand{\xone}{\rvx_1}
\newcommand{\xtwo}{\rvx_2}
\newcommand{\h}{\rvh}
\newcommand{\B}{\mathbf{\Phi}}
\newcommand{\Bone}{\rmB_1}
\newcommand{\Btwo}{\rmB_2}
\newcommand{\zone}{\rvz_1}
\newcommand{\ztwo}{\rvz_2}

\textbf{Data distribution~~} 
We consider binary classification and model 
the inputs as consisting of two kinds of features:
$x = [\xin, \xsp]$,
where $\xin \in \R^{\din}$ is the invariant feature 
that is predictive of the label
across both source $\ProbS$ and target $\ProbT$
and $\xsp \in \R^{\dsp}$ is the spurious feature 
that is correlated with the label $y$ 
only on the source domain $\ProbS$ 
but uncorrelated with label $y$ in $\ProbT$.
Formally, we sample $\ry \sim \unif \{-1, 1\}$ 
and generate inputs $x$ conditioned on $\ry$ as follows: 
\begin{align}
\footnotesize
\ProbS:~ \xin \sim  \sN(\gamma \cdot \ry \wstar, \Sigmain)~~\xsp = \ry \mathbf{1}_{\dsp}\,,~~  
\ProbT:~ \xin \sim \sN(\gamma \cdot \ry \wstar, \Sigmain)~~\xsp \sim \sN(\mathbf{0}, \Sigmasp), \label{eq:toy-setup}
\end{align}
where $\gamma$ is the margin afforded by the invariant feature. We set covariance of the invariant features $\Sigmain = \sigmain^2\cdot(\mathbf{I}_{\din} - {\wstar\wstar}^\top)$ to capture structure in the invariant feature that the variance is less along the latent predictive direction $\wstar$.
Note that the spurious feature is completely predictive
of the label in the source data,
and is distributed as Gaussian in the target data
with $\Sigmasp = \sigmasp^2 \mathbf{I}_{\dsp}$.
Our distribution shift setting bears similarities 
but also exhibits important differences 
(discussed in  \ref{app:toy_description}). 
For mathematical convenience,
we assume access to infinite unlabeled data
and hence replace the empirical quantities over unlabeled data 
with their population counterpart. 
For SSL, we sample finite labeled and infinite unlabeled data from $\ProbT$ where spurious features are absent (to exclude easy-to-generalize features).    
For UDA, we further assume access to infinite labeled data from the source. Note that due to distribution shift, population access of labeled data doesn't trivialize the problem as ``ERM'' on infinite labeled source data does not necessarily achieve optimal performance on the target. 




\textbf{Methods and objectives~~} Recall from Section~\ref{sec:problem-setup}
that we learn linear classifiers $h$ over features extractors $\Phi$.
We consider linear feature extractor i.e. $\Phi$ is a matrix in $\R^{d \times k}$ and
the linear layer $h: \R^k \to \R$ with a prediction as $\sgn(h^\top \Phi x)$. We use the exponential loss $\ell (f(x), y) = \exp\left(-y f(x)\right)$.


\textit{Self-training.} ST performs ERM
in the first stage using labeled data from the source,
and then subsequently updates the head $h$ 
by iteratively generating pseudolabels on the unlabeled target:
\begin{align}
\footnotesize
    \calL_\st(h; \Phi) \;\; & \coloneqq \;\; \Exp_{\ProbT(x)} \ell(h^\top \Phi x, \sgn(h^\top \Phi(x)))\qquad \nonumber \\
   \textrm{Update:}
   \;\; & h^{t+1}  \;\; = \;\; \frac{h^{t} - \eta \nabla_h \calL_\st (h^t; \Phi)}{\norm{h^{t} - \eta \nabla_h \calL_\st (h^t; \Phi)}{2}}
    \label{eq:self-training}
\end{align}
For ERM and ST, we train both $h$ and $\Phi$ (equivalent to $\Phi$ being identity and training a linear head). 

\textit{Contrastive pretraining.} We obtain $\Phi_\cl \coloneqq \argmin_\Phi \calL_\cl(\Phi)$ by minimizing the Barlow Twins objective~\citep{zbontar2021barlow}, 
which prior works have shown is also equivalent to spectral contrastive and non-contrastive objectives~\citep{garrido2022duality, cabannes2023ssl}. 
Given probability distribution $\ProbA(a \mid x)$ for input $x$,
and marginal $\ProbA$, 
we consider a constrained form of Barlow Twins
in \eqref{eq:cont-loss} which enforces 
features of ``positive pairs''  $a_1, a_2$
to be close while ensuring feature diversity.
We assume a strict regularization $(\rho=0)$ 
for the theory arguments in the rest of the paper, 
and in \appref{app:objectives} we prove that
all our claims hold for small $\rho$ as well.
For augmentations, we scale the magnitude 
of each co-ordinate uniformly by an independent amount, 
i.e., $a \sim \ProbA(\cdot \mid x) = \rvc \odot x $,
where $\rvc \sim \unif[0, 1]^d$. 
We try to mirror practical settings
where the augmentations are fairly ``generic'', 
not encoding information about which features 
are invariant or spurious, 
and hence perturb all features symmetrically. 
\begin{align}
    \footnotesize
    \calL_\cl(\Phi) \; \coloneqq & \; \Exp_{x \sim \ProbU}\Exp_{a_1, a_2 \sim \ProbA(\cdot \mid x)} \; \|\Phi(a_1) - \Phi(a_2)\|_2^2 \;\;\nonumber \\  \textrm{s.t.} & \;\; 
    \norm{\Exp_{a \sim \ProbA}\brck{\Phi(a)\Phi(a)^\top} - \mathbf{I}_k}{F}^2 \leq \rho
     \label{eq:cont-loss}
\end{align}
Keeping the $\Phi_\cl$ fixed, we then learn a linear classifier $h_\cl$ over $\Phi_\cl$ to minimize the exponential loss on labeled source data (refer to as \emph{linear probing}). 
For STOC, keeping the $\Phi_\cl$ fixed and initializing the linear head with the CL linear probe (instead of source only ERM), we perform ST with \eqref{eq:self-training}.














































\begin{example}\label{ex:toy_setup}
For the setup in \eqref{eq:toy-setup}, we choose $\gamma = 0.5$, $\sigmasp^2 = 1.$, and $\sigmain^2 = 0.05$ with $\din = 5$ and $\dsp=20$ for our running example. 
$\nicefrac{\gamma}{\sqrt{\dsp}}$ controls signal to noise ratio in the source such that spurious feature is easy-to-learn and the invariant feature is harder-to-learn. 
$\sigma_2$ controls the noise in target which we show later is critical in unlearning the spurious feature with CL.  
\end{example}

























\vspace{-5pt}
\subsection{Simulations and Intuitive Story: A Comparative Study Between SSL and DA}
\vspace{-5pt}
\label{subsec:intuitive-story}
\input{sections/toy-setup/simulation}

\vspace{-7pt}
\subsection{Conditions for Success and Failure of Self-training over ERM from Scratch}
\vspace{-5pt}

\label{subsec:self-training-analysis}

\input{sections/toy-setup/self-training}

\vspace{-5pt}
\subsection{CL Captures Both Features But Amplifies Invariant Over Spurious Features}
\vspace{-5pt}
\label{subsec:contrastive-pretraining-analysis}
\input{sections/toy-setup/contrastive-learning}



\vspace{-5pt}
\subsection{Improvements with Self-training Over Contrastive Learning}
\vspace{-5pt}
\label{subsec:combining-self-training-and-contrastive-pretraining}

\input{sections/toy-setup/combined}

\vspace{-5pt}
\subsection{Reconciling Practice: Implications for Deep Non-Linear Networks }
\vspace{-5pt}
\label{subsec:deep-networks}
\input{sections/toy-setup/deep}






































































 









==> sections/toyexperiments.tex <==
\section{Experiments on toy data}

\textbf{Setup.} Describe the following in the setup: 1) Data distribution for source, and target. 2) Contrastive-learning 
objective [should we analyze a non-contrastive loss like barlow twin or contrastive loss like simclr?] 3) Architecture used. 4) evaluation protocol (we fix backbone and train linear head).

\textbf{Parameters we fix for all ablations:} Before we generate plots, we need to fix some parameters: input dimension, $\|w^*\|_0$ or true dimensions, noisy dimensions, noise distribution, augmentation strength.  

\textbf{Results.} What plots do we want?
\begin{itemize}
    \item barplot: erm, fm, CL+ERM, CL+FM (4 bars in one block, different block for different contrastive learning losses)
    \item Contrastive learning LP performance as we vary odim (line plot, with one line for each contrastive loss).
    \item Show contrastive learning and contrastive learning + fixmatch performance, as we vary no of source samples and number of pre-training samples (should we do this for all three losses?). 
\end{itemize} 




